The sigma and f_0(980) from Ke4 + pi-pi scatterings data

We systematically reconsider, within an improved "analytic K-matrix model", the extraction of the sigma = f_0(600) and f_0(980) masses, widths and hadronic couplings using new Ke4 = K-->pi-pi e nu_e data on pi-pi phase shift below 390 MeV and different sets of pi-pi--> pi-pi / K-K scatterings data from 400 MeV to 1.4 GeV. Our results are summarized in Tables 1, 2 and 5. In units of MeV, the complex poles are: M_sigma=452(12) - i 260(15) and M_f=981(34) -i 18(11), which are comparable with some recent high-precision determinations and with PDG values. Besides some other results, we find: |g_{sigma K+K-}|/|g_{sigma pi+pi-}|=0.37(6) which confirms a sizeable g_{sigma K+K-} coupling found earlier, and which disfavours a large pi-pi molecule or four-quark component of the sigma, while its broad pi-pi width (relative to the one of the rho-meson) cannot be explained within a \bar qq scenario. The narrow pi-pi width of the f_0(980) and the large value: |g_{f K+K-}|/|g_{f pi+pi-}|=2.59(1.34), excludes its pure (\bar uu+\bar dd) content. A significant gluonium component eventually mixed with \bar qq appears to be necessary for evading the previous difficulties.

==> bib_sigmab.tex <==
%%%%%%%%%%%%%%%
\begin{thebibliography}{999}
\vspace*{-0.25cm}
%%%%%%%%%%%%%
% SCALARS
%%%%%%%%%%%%%
\bibitem{MONTANET} For reviews, see e.g.:
L. Montanet, {\it Nucl.
 Phys. Proc. Suppl.} {\bf 86},  (2000) 381; U. Gastaldi, {\it Nucl. Phys. Proc. Suppl.} {\bf 96},  (2001) 234;
 E. Klempt, A. Zaitsev, {\it Phys. Rept.} {\bf 454} (2007) 1; S.F. Tuan, {\it arXiv:hep-ph/0303248};  Different talks given at the sigma workshop, Kyoto (2000), ed. S. Ishida et al. 
 
 \bibitem{SN09} For a review, see e.g.: S. Narison, {\it Nucl. Phys. Proc. Suppl.} {\bf 186} (2009) 306.

\bibitem{MOUSSALAM}P. Buttiker, S. Descotes-Genon, B. Moussallam, {\it Eur. Phys. J.} {\bf C48} (2006)553.

%%%%%%%%%%%%%%%%
%  QUARK MODEL
%%%%%%%%%%%%%%%%

 \bibitem{MORGAN} D. Morgan,  {\it Phys. Lett.} {\bf B 51} (1974) 71.
 
  \bibitem{BN} A. Bramon and S. Narison, {\it Mod. Phys. Lett.} {\bf A 4}
 (1989) 1113.
 
\bibitem{SNG} S. Narison, {\it Nucl. Phys.} {\bf B 509} (1998) 312;  {\it Nucl. Phys. Proc. Suppl.} {\bf 64} (1998) 210;  {\it Nucl. Phys. Proc. Suppl.} {\bf 96} (2001) 244; {\it Nucl. Phys.} {\bf A 675} (2000) 54C;{\it Nucl. Phys. Proc.Suppl.}{\bf 121} (2003) 131.

\bibitem{KLEMPT} 
E. Klempt, B.C. Metsch, C.R. M$\ddot {\rm u}$nz and H.R. Petry,
{\it Phys. Lett.} {\bf B 361} (1995) 160.

\bibitem{OCHS}
P. Minkowski and W. Ochs, {\it  Eur. Phys. J.} {\bf  C
 9} (1999) 283.
 
 \bibitem{SN06} S. Narison, {\it Phys. Rev.} {\bf D 73} (2006) 114024.

%%%%%%%%%%%%%%%%%%
%  UNITARIZED QUARK MODEL
%%%%%%%%%%%%%%%%%%

 \bibitem{TORN}N. Tornqvist, {\it Phys. Rev. Lett.} {\bf 49} (1982) 624;
 {\it Z. Phys.} {\bf C 68} (1995) 467.
\bibitem{BEVEREN} E. van Beveren et al., {\it Z. Phys.} {\bf C 30} (1986)
615;  E. van Beveren and G. Rupp,  {\it Eur.Phys.J.} {\bf C 10} (1999) 469.

%%%%%%%%%%%%%%%%%
%  FOUR-QUARK STATES
%%%%%%%%%%%%%%%%%
\bibitem{JAFFE1}R. Jaffe, {\it Phys. Rev.} {\bf D 15} (1977) 267;  {\it
 Phys. Rev.} {\bf D 15} (1977) 281.
\bibitem{BLACK}J.M. Richard,  {\it Nucl. Phys. Proc. Suppl.} {\bf 164} (2005) 131;
D. Black et al., {\it Phys. Rev.} {\bf D 59} (1999)
 074026; A. Fariborz, R. Jora and J. Schechter, {\it Phys. Rev.} {\bf D 79} (2009) 074014; D. Wong and K.F. Liu, {\it Phys. Rev.} {\bf D 21} (1980) 2039; 
M. Alford and R.L. Jaffe, {\it Nucl. Phys.} {\bf B 509} (1998) 312; 
F. Buccella et al., {\it Eur. Phys. J.} {\bf C~49} (2007) 743;
M. Karliner, H. J. Lipkin, {\it Phys. Lett.} {\bf B 612} (2005) 197;
L. Maiani et al., {\it Phys. Rev. Lett.} {\bf  93} (2004) 212002;
A. Selem and F.Wilczek, hep-ph/0602128; S. Prelovsek et al., 
{ \it arXiv : 1002.0193 [hep-ph]} (2010). 
\bibitem{LATORRE}J.I. Latorre and P. Pascual, {\it Jour. Phys. } {\bf G 11} (1985) L231;
T.V. Brito et al., {\it Phys. Lett.} {\bf  B 608} (2005) 69; R.D. Matheus et al., {\it Phys. Rev.} {\bf D 76} (2007) 056005.
\bibitem{SNA0} S. Narison, {\it Phys. Lett.} {\bf B 175} (1986) 88.
\bibitem{ACHASOV}N.N. Achasov, S.A. Devyanin and G.N. Shestakov, {\it
 Z. Phys.} {\bf C 16} (1984) 55; N.N. Achasov,{\it Nucl. Phys. Proc. Suppl.} {\bf 186} (2009) 283; C. Hanhart et al., {\it hep-ph / 0701214} (2007).
 %%%%%%%%%%%%%%
 %  MOLECULES
 %%%%%%%%%%%%%
\bibitem{ISGUR}N. Isgur and J. Weinstein, {\it Phys. Rev.} {\bf D 41}
 (1990) 2236.
\bibitem{BARNES} T. Barnes,  {\it Phys. Lett.} {\bf B 165} (1985) 434;
 Proc. IXth Int. Workshop on $\gamma\gamma$ collisions, World Scientific
 (1992) 263 ed. D. Caldwell and H.P. Paar.
 %%%%%%%%%%%%%%
 % MESON EXCHANGE
 %%%%%%%%%%%%%%
\bibitem{HOLINDE}G. Janssen et al., {\it Phys. Rev.} {\bf D 52} (1995)
 2690.
 %%%%%%%%%%%%%%%%
 % GLUEBALL
 %%%%%%%%%%%%%%%%
 \bibitem{MIN} H. Fritzsch, P. Minkowski, {\it Nuovo Cimento} {\bf A  30} (1975) 393.

 \bibitem{VENTO}V. Crede, C.A. Meyer, 
 {\it arXiv: 0812.0600 [hep-ex] } (2008); V. Mathieu , N. Kochelev, V. Vento, { \it arXiv : 0810.4453 [hep-ph]} (2008). 
 %%%%%%%%%%%%%%%%%%
% GLUEBALLS PHENOMENOLOGY 
%%%%%%%%%%%%%%%%%%%
\bibitem{MINK} P. Minkowski, W. Ochs, {\it  Eur. Phys. J.} {\bf  C
 9} (1999) 283;  {\it Nucl. Phys. Proc. Suppl.} {\bf 121} (2003) 119; 
{\it  ibid} {\bf 121} (2003) 121; {\it  Eur. Phys. J.} {\bf  C
 39} (2005) 71; W. Ochs, {\it Nucl. Phys. Proc. Suppl.} {\bf 174} (2007) 146.
 
 \bibitem{OLLER} M. Albaladejo and J.A. Oller, {\it Phys. Rev. Lett.}  {\bf 101} (2008) 252002; D. V. Bugg, M. J. Peardon and B. S. Zhou, {\it Phys. Lett.} {\bf B 486} (2000) 49.
 
 \bibitem{CHANOW} M.S.Chanowitz, {\it Phys. Rev. Lett.}  {\bf 95} (2005) 172001; {\bf 98} (2007) 149104.

 %%%%%%%%%%%%%%%%
% GLUEBALL LATTICE
%%%%%%%%%%%%%%%%
\bibitem{PEARDON}  C.  Morningstar and  M.  J.   Peardon ,
 {\it Phys. Rev.} {\bf D 60} (1999) 034509;
  G. Bali et al.,  {\it Phys. Rev.}  {\bf D 62} (2000)
 054503;  A. Hart and M. Teper, {\it Phys. Rev.}  {\bf D 65} (2002) 34502; Y.
 Chen et al., {\it Phys. Rev.} {\bf D 74} (2006) 094005; ; H. Wada et
 al. , {\it Phys. Lett.} {\bf B 652} (2007) 250.
%  \bibitem{MICHAEL}A. Hart et al., 
%  {\it Phys. Rev.} {\bf D 74} (2006) 114504; 
  %C. Michael et al. , hep-lat/9909036; 
T. Kunihiro et al., {\it Phys. Rev.} {\bf D
 70} (2004) 034504. 
 
  \bibitem{MICHAEL}A. Hart et al.,   {\it Phys. Rev.} {\bf D 74} (2006) 114504; C. McNeile, {\it Nucl. Phys. Proc. Suppl.} {\bf 186} (2009) 264.  
  
\bibitem{FRASCA}M. Frasca, {\it Nucl. Phys. Proc. Suppl.} {\bf 186} (2009) 260; {\it arXiv: 0812.0934 [hep-ph].}
%%%%%%%%%%%%%%%%%%
% QSSR GLUEBALL 
%%%%%%%%%%%%%%%%%%
\bibitem{NSVZ}V.A. Novikov et al., {\it Nucl. Phys.} {\bf B 191} (1981)
 301.
 
 \bibitem{CHET} K. Chetyrkin, S. Narison and V.I. Zakharov, {\it Nucl. Phys.} {\bf B 550} (1999)
353.

\bibitem{SNG0}S. Narison, {\it Z. Phys.} {\bf  C 22} (1984) 161.
\bibitem{SNG1} P. Pascual and R. Tarrach, {\it Phys. Lett.} {\bf B 113} (1982) 495;
S. Narison, {\it Phys. Lett.} {\bf B 125} (1983) 501;
C.A. Dominguez and N. Paver,   {\it Z. Phys.} {\bf  C 31} (1986) 591;
J. Bordes, V. Gimenez and J.A. Pe\~narrocha,  {\it Phys. Lett.} {\bf B 223} (1989) 251;
E. Bagan and T.G.  Steele,  {\it Phys. Lett.} {\bf B 243} (1990) 413; 
J.L. Liu and D. Liu, {\it J. Phys} {\bf G 19} (1993) 373; L.S. Kisslinger, J. Gardner
and C. Vanderstraeten,  {\it Phys. Lett.} {\bf B 410} (1997) 1; T. Huang, H.Y. Jin and A.L.  Zhang,
 {\it Phys. Rev.} {\bf D 58} (1998) 312;
D. Harnett, K. Moats, T.G. Steele, {\it arXiv: 0804.2195 [hep-ph].};
T.G. Steele, D. Harnett and G. Orlandini, {\it AIP Conf. Proc.} {\bf  688} (2004); H. Forkel, {\it Phys. Rev.} {\bf D 71} (2005) 054008. 
\bibitem{VENEZIA} S. Narison and G. Veneziano, {\it Int. J. Mod. Phys.}
 {\bf A 4} (1989) 2751.
 %%%%%%%%%%%%%%%%%%%
% QSSR SVZ & REVIEW
%%%%%%%%%%%%%%%%%%%
\bibitem{SVZ}M.A. Shifman, A.I. Vainshtein and V.I. Zakharov,
{\it Nucl. Phys.} {\bf B 147} (1979) 385, 448.

\bibitem{SNB}For reviews, see e.g.: S. Narison, {\it 
%QCD as a theory of hadrons,
Cambridge Monogr. Part. Phys. Nucl. Phys. Cosmol.} {\bf 17}
 (2004) 1-778 [hep-ph/0205006]; {\it World Sci. Lect. Notes Phys.} {\bf 26} (1989) 1-527; 
{\it Acta Phys. Pol.} {\bf 26} (1995) 687;  {\it Riv. Nuov.
 Cim.} {\bf 10 N2} (1987) 1;  {\it Phys. Rep.}  {\bf 84} (1982) . 
 
 %%%%%%%%%%%%%
%LOW-ENERGY THEOREMS
%%%%%%%%%%%%
\bibitem{NOVIKOV}V.A. Novikov et al., {\it Nucl. Phys.} {\bf B 165} (1980) 67.

\bibitem{CHANO}R.J. Crewther, {\it Phys. Rev. Lett.} {\bf  28} (1972) 1421; J. Ellis and M.S. Chanowitz,
{\it Phys. Lett.} {\bf B 40} (1972) 397;  {\it Phys. Rev. } {\bf  D 7} (1973) 2490.

%%%%%%%%%%%%%%%
% AdS/QCD
%%%%%%%%%%%%%%%
\bibitem{HERY}P. Colangelo et al.,  {\it Phys. Lett.} {\bf B 652} (2007) 73; H. Forkel, {\it Phys. Rev. } {\bf  D 78} (2008) 055009; H. Ratsimbarison, {\it arXiv: 0911.4553 [hep-ph]} (2009).
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
% LARGE N_c
%%%%%%%%%%%%%%%%
\bibitem{PELAEZ}J.R. Pelaez, {\it Phys. Rev. Lett.} {\bf 92} (2004) 102001; J. Ruiz de Elvira et al., {\it arXiv: 1001.2746 [hep-ph]} (2010).

\bibitem{ARRIOLA} E. Ruiz Arriola and W. Broniowski, {\it arXiv: 1001.1636 [hep-ph]} (2010).

%%%%%%%%%%%%%%%%
% MESON-GLUONIUM MIXING
%%%%%%%%%%%%%%%%
\bibitem{CLOSE} C. Amsler and F.E. Close, {\it Phys. Rev.} {\bf D 53}
 (1996) 295;
D. Weingarten, {\it Nucl. Phys. Proc. Suppl.} {\bf 73}
 (1999) 283; 
%C. Amsler, hep-ph/0206104; 
F.E. Close and A. Kirk, {\it Eur.Phys.J.} {\bf C 21} (2001) 531;
%hep-ph/0103173; 
F. Giacosa et al.,
 {\it Phys. Lett.} {\bf B 622} (2005) 277;
% hep-ph/0504033; 
X.G. He et al., {\it Phys. Rev.} {\bf D
 73} (2006) 114026;
F.E. Close and Q. Zhao,   {\it Phys. Rev.} {\bf D 71} (2005) 094022.
%V. Anisovich, Yu. Prokoshkin and A. Sarantsev,  {\it Phys. Lett.} {\bf B 389} (1996) 388.
\bibitem{aniso}V. Anisovich, Yu. Prokoshkin and A. Sarantsev, 
 {\it Phys. Lett.} {\bf B 389} (1996) 388.
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{LANIK} J. Ellis and J. Lanik,  {\it Phys. Lett.} {\bf B
 150} (1985) 289;  {\it Phys. Lett.} {\bf B 175} (1986) 83; J.Lanik, {\it Z. Phys.} {\bf C 39} (1988) 143.

\bibitem{SCHEC}P. Di Vecchia and G. Veneziano, {\it Nucl. Phys.} {\bf
 B 171} (1980) 253;  P. Jain, R. Johnson and J. Schechter, {\it Phys. Rev.} {\bf D 35} (1987) 2230.

\bibitem{ZHENG}L. Y. Xiao, H. Q. Zheng and Z. Y. Zhou,  {\it Nucl. Phys. Proc. Suppl.} {\bf 174} (2007) 142.

\bibitem{PICH} G. Ecker et al., {\it Nucl. Phys.} {\bf B321} (1989) 31.

\bibitem{CHANFRAY}M. Ericson and G. Chanfray, {\it AIP Conf. Proc.} {\bf 1030} (2008) 13; {\it Eur. Phys. J.} {\bf A 34} (2007) 215. 

%%%%%%%%%%%%%%%
% K-MATRIX \gamma\gamma
%%%%%%%%%%%%%%%
\bibitem{MNO} G. Mennessier, S. Narison, W. Ochs, {\it Phys. Lett.} {\bf B 665} (2008) 205; 
{\it Nucl. Phys. Proc. Suppl.} {\bf 238} (2008) 181; 
G. Mennessier, P. Minkowski, S. Narison, W. Ochs, HEPMAD 07 Conference,  SLAC Econf  C0709107, {\it arXiv: 0707.4511 [hep-ph] } (2007).

%%%%%%%%%%%%
% GLUEBALLS
%%%%%%%%%%%%

%%%%%%%%%%%%%
% K-MATRIX
%%%%%%%%%%%%%
\bibitem{KMN}R. Kaminski, G. Mennessier and S. Narison, {\it Phys. Lett.} {\bf B 680} (2009) 148.

%%%%%%%%%%%%%%%%%%
% NEW DATA
%%%%%%%%%%%%%%%%%
\bibitem{NA48} The NA48/2 collaboration: B. Bloch-Devaux, {\it PoS Confinement8} (2008) 029; J.R. Batley et al., {\it Eur. Phys. J. }{\bf C 52} (2007) 875-891.

%%%%%%%%%%%%%%
% DATA pi-pi 
%%%%%%%%%%%%%
\bibitem{MUNICH} G. Grayer et al.,  {\it Nucl. Phys.} {\bf B 75} (1974) 189.

\bibitem{HYAMS} B. Hyams et al., {\it Nucl. Phys.} {\bf B 64}
 (1973) 134; W. Ochs, Univ. Munich Thesis (1974).

\bibitem{COHEN} D. Cohen et al., {\it Phys. Rev.} {\bf D 22} (1980) 2595.

\bibitem{ETKIN} A. Etkin et al. {\it Phys. Rev.} {\bf D 25} (1982) 1786; A.D. Martin and E.N. Ozmultu,
{\it Nucl. Phys.} {\bf B 158} (1979) 5201.

\bibitem{KLL} R. Kaminski,  L. Lesniak and B. Loiseau , {\it Phys. Lett.} {\bf B 413} (1997) 130; {\it Eur. Phys. J} {\bf C 9} (1999) 141; R. Kaminski, L. Lesniak, K. Rybicki, {\it Z. Phys.} {\bf  C 74} (1997) 79. 
%\bibitem{BELLE} The Belle collaboration: T. Mori et al. {\it Phys. Rev.} {\bf D 75} (2007) 051101 [hep-ex/0610038];  {\it J. Phys. Soc. Jap.} {\bf 76} (2007) 074102 [arXiv: 0704.3538].

%%%%%%%%%%%%%
% K-MATRIX ORIGINAL
%%%%%%%%%%%%%
\bibitem{MENES} G. Mennessier, {\it Z. Phys.} {\bf  C 16} (1983) 241;
O. Babelon et al., {\it Nucl. Phys.} {\bf B 113} (1976) 445.
\bibitem{PEAN} G. Mennessier, T.N. Truong, {\it Phys. Lett.} {\bf B 177} (1986) 195;
A Pean, Th\` ese  Montpellier (1992) (unpublished).

%%%%%%%%%%%
% ASYMMETRY
%%%%%%%%%%%
\bibitem{LAYSSAC}J. Layssac, S. Narison, {\it Nucl. Phys. Proc.Suppl} {\bf 186} (2009) 203.

%%%%%%%%%%%%%
% CGL
%%%%%%%%%%%%%
\bibitem{leutwyler} I. Caprini, G. Colangelo and H. Leutwyler,  {\it
  Phys. Rev. Lett.} {\bf 96} (2006) 132001; {\it Phys. Rev.} {\bf D 68} (2003) 074005.


%%%%%%%%%%%%%
% SIGMA MASS
%%%%%%%%%%%%%
  
\bibitem{GKPY}  R. Kaminski, J.R. Pelaez and F.J. Yndurain,
{\it Phys. Rev.} {\bf D 77} (2008) 054015; F.J. Yndurain , R. Garcia-Martin, J.R. Pelaez,
{\it Phys. Rev.} {\bf D 76} (2007) 074034. 


\bibitem{BES2}M. Ablikim et al., {\it Phys. Lett.} {\bf B 598} (2004) 149.

\bibitem{E741}E.M. Aitala et al., {\it Phys. Rev. Lett.} {\bf 86} (2001) 770.

\bibitem{MINKOWSKI} P. Minkowski, {\it Nucl. Phys. Proc. Suppl.} {\bf 186} (2009) 302; P. Minkowski and A. Schenk, {\it Nucl. Phys.} {\bf B 363} (1991) 97.

\bibitem{ACHA}N.N. Achasov and A.V. Kiselev, {\it arXiv:hep-ph/0512047} (2006).

%%%%%%%%%%%%
% PDG
%%%%%%%%%%%%
\bibitem{PDG}PDG, C. Amsler et al., {\it Phys. Lett.} {\bf B 667} (2008) 1.

%%%%%%%%%%%%%%%%%%%%%
% MODELS
%%%%%%%%%%%%%%%%%%%%%
\bibitem{WANG}Yu. Mao, X-G. Wang, O. Zhang, H-Q. Zheng, Z-Y. Zhou, {\it Phys. Rev.} {\bf D 79} (2009) 116008.

\bibitem{BUGG}D.V. Bugg, {\it Eur. Phys. J.} {\bf C 47} (2006) 45.
% and private communications.

\bibitem{BES}M. Ablikim et al.,  {\it Phys. Lett.} {\bf B 607} (2005) 243.

%%%%%%%%%%%%%%%%%%%%%%%%%%
% ON SHELL MASS AND BREIT WIGNER
%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{SIRLIN}B.A. Kniehl, A. Sirlin,  {\it Phys. Rev.} {\bf D 77} (2008) 116012.

\bibitem{ESTABROOKS} P. Estabrooks,  {\it Phys. Rev.} {\bf D 19} (1979)
2678. 

\bibitem{AMP} K.L. Au, D. Morgan, M. Pennington, 
    {\it Phys. Rev.} {\bf D 35} (1987) 1633.

%%%%%%%%%%%%%%%%%%%%%
% GLUON CONDENSATE
%%%%%%%%%%%%%%%%%%%%%
\bibitem{SNHeavy} S. Narison, {\it Phys. Lett.} {\bf B 387} (1996) 162.
\bibitem{LNT} G. Launer, S. Narison and R. Tarrach, {\it Z. Phys.} {\bf C 26} (1984) 433.
\bibitem{SNI}S. Narison, {\it Phys. Lett.} {\bf B 300} (1993) 293; ibid {\bf B 361} (1995) 121.
\bibitem{SNTAU}S. Narison, {\it Phys. Lett.} {\bf B 673} (2009) 30.
%%%%%%%%%%%%%%%%%%%%
% GLUEBALL TESTS
%%%%%%%%%%%%%%%%%%%%
\bibitem{DOSCH} H.G. Dosch and S. Narison, {\it Nucl. Phys. Proc. Suppl.} {\bf 121} (2003) 114.

\end{thebibliography}
\end{document}














%%%%%%%%%%%%%%%%
% QSSR GLUEBALL
%%%%%%%%%%%%%%%
\bibitem{SNG0}S. Narison, {\it Z. Phys.} {\bf  C 26} (1984) 209.

\bibitem{VENEZIA} S. Narison, G. Veneziano, {\it Int. J. Mod. Phys.}
 {\bf A 4} (1989) 2751.
 
\bibitem{SN06} S. Narison, {\it Phys. Rev.} {\bf D 73} (2006) 114024.

\bibitem{STEELE}D. Harnett, K. Moats, T.G. Steele, {\it arXiv: 0804.2195 [hep-ph].}
%; H. Forkel, {\it Phys. Rev.} {\bf D 71} (2005) 054008.



%%%%%%%%%%%%%%%%%
%  QQ  MIXING
%%%%%%%%%%%%%%%%%
 
\bibitem{SNHYB} For a review, see e.g., S. Narison, {\it Nucl. Phys.} {\bf A 675} (2000) 54c.

\bibitem{DOSCHGLUE} H. G. Dosch, S. Narison, {\it Nucl. Phys. Proc. Suppl. } {\bf 121} (2003)114.

\bibitem{CLOSE} C. Amsler, F.E. Close, {\it Phys. Rev.} {\bf D 53}
 (1996) 295; F. E. Close, Q. Zhao, {\it Phys. Rev.}  {\bf D 71}  (2005) 094022. 


%%%%%%%%%%%%
%2gamma
%%%%%%%%%%%%
\bibitem{PENNINGTON}M.R. Pennington, {\it Phys. Rev. Lett.} {\bf 97} (2006)011601 and
 {\it Mod. Phys. Lett.} {\bf A 22} (2007) 1439; 
M. Boglione, M.R. Pennington, {\it Eur.Phys.J.} {\bf C9} (1999) 11.

\bibitem{PENN1}M.R. Pennington, T. Mori, S. Uehara and Y. Watanabe,
{\it Eur. Phys. J.} {\bf C 56} (2008) 1.

\bibitem{OLLER}J.A. Oller, L. Roca, C. Schat, {\it Phys. Lett.} {\bf B
 659} (2008) 201; J.A. Oller, L. Roca, {\it Eur. Phys. J.} {\bf A 37} (2008) 15.
 
\bibitem{PRADES}J. Bernabeu, J. Prades, {\it Phys. Rev. Lett.} {\bf 100} (2008) 241804;
{\it arXiv:0809.2475 [hep-ph] }. 

\bibitem{ZHENG09}Yu. Mao, X-G. Wang, O. Zhang, H-Q. Zheng, Z-Y. Zhou, {\it  arXiv:0904.1445 [hep-ph]}; Z-G. Xiao, H-Q. Zheng, {\it Commun. Theor. Phys. (Beijing, China)} {\bf 48} (2007) 685.
%%%%%%%%%%%
% pi-pi to pi-pi
%%%%%%%%%%%
\bibitem{leutwyler} I. Caprini, G. Colangelo and H. Leutwyler,  {\it
  Phys. Rev. Lett.} {\bf 96} (2006) 132001; {\it Phys. Rev.} {\bf D 68} (2003) 074005.
  
\bibitem{GKPY}  R. Kaminski, J.R. Pelaez and F.J. Yndurain,
{\it Phys. Rev.} {\bf D 77} (2008) 054015; F.J. Yndurain , R. Garcia-Martin, J.R. Pelaez,
{\it Phys. Rev.} {\bf D 76} (2007) 074034. 

\bibitem{BES2}M. Ablikim et al., {\it Phys. Lett.} {\bf B 598} (2004) 149.

\bibitem{E741}E.M. Aitala et al., {\it Phys. Rev. Lett.} {\bf 86} (2001) 770.

 %%%%%%%%%%%%%%%%%%%
% QSSR SVZ & REVIEW
%%%%%%%%%%%%%%%%%%%
\bibitem{SVZ}M.A. Shifman, A.I. Vainshtein and V.I. Zakharov,
{\it Nucl. Phys.} {\bf B 147} (1979) 385, 448.

\bibitem{SNB}For reviews, see e.g.: S. Narison, {\it 
%QCD as a theory of hadrons,
Cambridge Monogr. Part. Phys. Nucl. Phys. Cosmol.} {\bf 17}
 (2004) 1-778 [hep-ph/0205006]; S. Narison, {\it World Sci. Lect. Notes Phys.} {\bf 26} (1989) 1-527; 
S. Narison, {\it Acta Phys. Pol.} {\bf B 26} (1995) 687;  
%S. Narison, {\it Riv. Nuovo Cim.} {\bf 10 N2} (1987) 1;  
 S. Narison, {\it Phys. Rept.}  {\bf 84} (1982) 263. 
 
 %%%%%%%%%%%%%
%LOW-ENERGY THEOREMS
%%%%%%%%%%%%
\bibitem{NOVIKOV}V.A. Novikov et al., {\it Nucl. Phys.} {\bf B 165} (1980) 67.

\bibitem{CHANO}R.J. Crewther, {\it Phys. Rev. Lett.} {\bf  28} (1972) 1421; J. Ellis, M.S. Chanowitz,
{\it Phys. Lett.} {\bf B 40} (1972) 397;  {\it Phys. Rev. } {\bf  D 7} (1973) 2490; P. Di Vecchia, G. Veneziano, {\it Nucl. Phys.} {\bf B 171}
(1981) 253.

%%%%%%%%%%%%%%%%%
%  QQ  AND 2-PHOTON WIDTH
%%%%%%%%%%%%%%%%%
\bibitem{SNA0} S. Narison, {\it Phys. Lett.} {\bf B 175} (1986) 88.
\bibitem{SNMENES}G. Mennessier, S. Narison, N. Paver, {\it Phys. Lett.} {\bf B 158} (1985) 153.
\bibitem{ROSNER}J. Babcock, J.L. Rosner, {\it Phys. Rev.} {\bf D 14} (1976) 1286.
\bibitem{LANIK}J.Ellis,  J. Lanik, {\it Phys. Lett.} {\bf B 150} (1985) 289.
\bibitem{BARNES}T. Barnes,  {\it Phys. Lett.} {\bf B 165} (1985) 434.
%%%%%%%%%%%%%%
% 4 QUARK
%%%%%%%%%%%%%%

\bibitem{LATORRE}J.I. Latorre, P. Pascual, {\it Jour. Phys. } {\bf G 11} (1985) L231;
M. Nielsen, R.D. Matheus, F.S. Navarra, {\it Nucl. Phys. Proc. Suppl.} {\bf 174} (2007) 138;
T.V. Brito, F.S. Navarra, M. Nielsen, M.E. Bracco, {\it Phys. Lett.} {\bf  B 608} (2005) 69; R.D. Matheus, F.S. Navarra, M. Nielsen, R. Rodrigues da Silva , {\it Phys. Rev.} {\bf D 76} (2007) 056005.
\bibitem{ACHASOV}N.N. Achasov, S.A. Devyanin and G.N. Shestakov, {\it
 Z. Phys.} {\bf C 16} (1984) 55; C. Hanhart, Yu. S. Kalashnikova, A. E. Kudryavtsev, A. V. Nefediev,  {\it Phys. Rev.} {\bf D 75} (2007) 074015; T.Barnes, 
Proc. IXth Int. Workshop on photon-photon collision (San Diego, 1992), ed. D. Caldwell and H.P. Paar (World Scientific, 1992), p. 263.

%%%%%%%%%%%%%%
% DATA pi-pi 
%%%%%%%%%%%%%
\bibitem{HYAMS} B. Hyams et al., {\it Nucl. Phys.} {\bf B 64}
 (1973) 134;
G. Grayer et al.,  {\it Nucl. Phys.} {\bf B 75} (1974) 189; Ochs, Univ. Munich Thesis (1974).

\bibitem{COHEN} D. Cohen et al., {\it Phys. Rev.} {\bf D 22} (1980) 2595.

\bibitem{ETKIN} A. Etkin et al. {\it Phys. Rev.} {\bf D 25} (1982) 1786.

%%%%%%%%%%%%%
% K-MATRIX
%%%%%%%%%%%%%
\bibitem{GKPYconf}  J.R. Pelaez, R. Garcia-Martin, R. Kaminski, F.J. Yndurain, {\it Nucl. Phys. Proc. Suppl.} {\bf 186} (2009) 312; R. Kaminski, R. Garcia-Martin, P. Grynkiewicz, J.R. Pelaez, {\it Nucl. Phys. Proc. Suppl.} {\bf 186} (2009) 318.

\bibitem{KLL} R. Kaminski,  L. Lesniak and B. Loiseau , {\it Phys. Lett.} {\bf B 413} (1997) 130; {\it Eur. Phys. J} {\bf C 9} (1999) 141. 

\bibitem{KLR} R. Kaminski, L. Lesniak, K. Rybicki, {\it Z. Phys.} {\bf  C 74} (1997) 79.

\bibitem{PYI} J. R. Pelaez and F. J. Yndurain, {\it Phys. Rev.} {\bf  D 71} (2005) 074016.

%%%%%%%%%%%%%%
% MODELS
%%%%%%%%%%%%%
\bibitem{ZHENG2}Z-G. Xiao, H-Q. Zheng, {\it Commun. Theor. Phys. (Beijing, China)} {\bf 48} (2007) 685; Z-G. Xiao, H. Q. Zheng, Z. Y. Zhou, {\it Nucl. Phys. Proc. Suppl.} {\bf 174} (2007) 142.


\bibitem{BUGG}D.V. Bugg, {\it Eur. Phys. J.} {\bf C 47} (2006) 45.
% and private communications.

\bibitem{BES}M. Ablikim et al.,  {\it Phys. Lett.} {\bf B 607} (2005) 243.

%%%%%%%%%%%%%%%%%

 \bibitem{GAMS}  D. Alde et al., Eur. Phys. J. A3 (1998) 361.
 

\bibitem{CHANOW}M.S.Chanowitz, {\it Phys. Rev. Lett.} {\bf 95} (2005) 172001.


%%%%%%%%%%%%%%%%%%%
%  U(1) ANOMALY
%%%%%%%%%%%%%%%%%%%
\bibitem{WITTEN}E. Witten, {\it Nucl. Phys} {\bf B156} (1979) 269; 
G. Veneziano,
 {\it Nucl. Phys.} {\bf B159} (1979) 213; A. Di Giacomo, {\it Nucl. Phys. Proc. Suppl.} {\bf B 23} (1991) 191;
S. Narison, {\it Phys. Lett.} {\bf B 125} (1983) 501.

\bibitem{PELAEZ} J.R. Pelaez, G. Rios, {\it Phys. Rev. Lett.} {\bf 97} (2006) 242002.

\bibitem{VENEZIANO}G. Veneziano, {\it Nucl. Phys.} {\bf B 117} (1976) 519.

\bibitem{MOUSSALAM}P. Buttiker, S. Descotes-Genon, B. Moussallam, {\it Eur. Phys. J.} {\bf C48} (2006)553.

\bibitem{SCHECHTER} R. Jaffe, {\it Phys. Rev.} {\bf D 15} (1977) 267; A.M. Fariborz, R. Jora, J. Schechter, {\it Nucl. Phys. Proc. Suppl.} {\bf 186} (2009) 298; G. t'Hooft, G. Isidori, L. Maiani, A.D. Polosa, V. Riquer, {\it Phys. Lett.} {\bf B 662} (2008) 424; J.M. Richard,  {\it Nucl. Phys. Proc. Suppl.} {\bf 164} (2005) 131; D. Black et al., {\it Phys. Rev.} {\bf D 59} (1999) 074026.

\bibitem{SNQ}For reviews, see e.g.: S. Narison, {\it Phys.Rev.} {\bf D 74}, 034013 (2006); {\it arXiv:hep-ph 0202200}; {\it Nucl. Phys. Proc. Suppl.} {\bf 86},  242 (2000); {\it Riv. Nuovo Cim.} {\bf 10N2}, 1 (1987).

\bibitem{SCAL}S. Narison, N. Paver, E. de Rafael, D. Treleani, {\it Nucl. Phys.} {\bf B 212} (1983) 365;  M.~Jamin, J.A.~Oller, A.~Pich, {\it Eur.\ Phys.\ J.} \ {\bf C 24} (2002) 237.

\end{thebibliography}
\end{document}



